Learning Curves for Analysis of Deep Networks

Learning curves model a classifier's test error as a function of the number of training samples. Prior works show that learning curves can be used to select model parameters and extrapolate performance. We investigate how to use learning curves to evaluate design choices, such as pretraining, architecture, and data augmentation. We propose a method to robustly estimate learning curves, abstract their parameters into error and data-reliance, and evaluate the effectiveness of different parameterizations. Our experiments exemplify use of learning curves for analysis and yield several interesting observations.

==> 02_related_work.tex <==
\section{Related Work}
\label{sec:related}

\boldhead{Learning curves}



Learning curves were first introduced in 1993 by Cortes et al.~\cite{cortes_nips1993_learning_curves} to speed up CNN model selection, but few studies in computer vision have evaluated error as a function of training size (e.g.~\cite{sun_iccv2017_unreasonable_effectiveness,hestness_2017arxiv_deeplearningpredictable}). To our knowledge, learning curves have not yet been used to compare approaches or understand impact of design decisions. 

\boldhead{Bias-variance tradeoff}

The bias-variance trade-off~\cite{geman_1992neural_biasvariance,domingo_icml2000_biasvariance} is an intuitive and theoretical way to think about generalization.  The ``bias'' is error due to inability of the classifier to encode the optimal decision function, and the ``variance'' is error due to variations in predictions caused using limited training samples for parameter estimation.  This is termed a trade-off because a classifier with more parameters may tend to have less bias but higher variance. Theoretically, the total error can be modeled as $error_N^2 = bias^2 + noise^2 + variance$, where ``noise'' is irreducible error due to non-unique mapping from inputs to labels, and variance can be modeled as $variance=\sigma^2/N$ for $N$ data points.


Recent works (e.g.~\cite{sun_iccv2017_unreasonable_effectiveness}) often claim a log-linear relationship between error and training size, but this holds only when asymptotic error is zero.  The relationship is better characterized as $error = a + b N^\gamma$, where $a$ is the asymptotic error reached when the number of samples $N=\infty$ and $b$ indicates the sensitivity of learning to the number of samples. Theory predicts $\gamma=0.5$, as can be seen by the bias-variance trade-off~\cite{geman_1992neural_biasvariance} extended to classification by Domingo~\cite{domingo_icml2000_biasvariance}: $error_N^2 = bias^2 + noise^2 + variance$, where bias is the error due to inability of the classifier to fit the optimal function, noise is intrinsic error due to a non-unique mapping from inputs to labels, and variance is the change in predictions across samples that occurs for different models sampling $N$ data points which can be modeled as $variance=\sigma^2/N$. Likewise, many generalization bound theorems can be simplified into the form $error = a + b / \sqrt{N}$, with $b$ typically involving many terms that relate to the complexity of the classifier. Hestness et al.~\cite{hestness_2017arxiv_deeplearningpredictable} show that when hyperparameters are not well tuned $\gamma < 0.5$ empirically, but our preliminary experiments (Fig.~\ref{fig:learning_curves}) show a good fit to $error = a + b N^\gamma$.    

\boldhead{Generalization theory}
The ability of a model to generalize can be measured by generalization error which is defined as the difference between train and test error. Statistical learning has developed several measures of capacity (or complexity measure of a hypothesis class) that can be used provide bounds on the generalization error. VC-dimension is equal to the largest number of data samples, $N$, that a hypothesis class can 'shatter', which means that some set of parameters exist for the function to correctly classifies all samples for all corresponding labels. The generalization bound developed using VC-dimension states that the generalization error is on the order of $O(\sqrt{\frac{H_{VC}}{m}})$, where $H_{VC}$ is the VC-dimension of the hypothesis class and $m$ is the size of the training set.\cite{vapnik:264} Another metric for computing is Rademacher Complexity. The empirical Rademacher complexity of a hypothesis class $H$ on a dataset ${x_1,\dots,x_n}$ drawn from distribution $D$ is defined as $\hat{R}_{S}(H) = E_{\sigma}\left[ sup_{h \in H} \frac{1}{n} \sum_{i = 1}^{n} \sigma_i h(x_i) \right]$ where $\sigma_1, \dots, \sigma_n \in {\pm 1}$. Rademacher complexity is the expectation of empirical Rademacher complexity: for any integer $m \leq 1$, the Rademacher complexity of $H$ with respect to sample size $n$ drawn from distribution $D$ is $R(H) = E_{S\thicksim D^n}[R_S(H)]$. The corresponding generalization bound states that generalization error is bounded by $2*R(H) + O(\frac{1}{\sqrt{m}})$.


While both VC-dimension and Rademacher complexity have been used as complexity measures for some hypothesis classes, it has not been shown that these complexity measures lead to tight generalization bounds that explain the low generalization error produced by deep neural networks. Key experiments conducted in \cite{zhangBHRV16} showed that deep neural networks can easily fit randomly labeled training data which leads to both generalization bounds based on VC-dimension and Rademacher complexity to be trivial. \cite{zhangBHRV16}

In the past few years, there has been work done developing new ways to measure complexity. Most of the bounds that result from these new measures usually are of the form $O\left(\sqrt{\frac{c^{x}}{m}}\right)$, where $c$ is some measure of complexity, $x$ is some exponent greater than $1$ and $m$ is the number of training examples.  Several bounds have been developed that use margin bounds and different measures of norms. In \cite{neyshabur2018a}, a generalization bound is developed that relies on the number of layers in the neural network:
\[
O\left(\sqrt{\frac{B^2d^2hln(dh)\pi_{i=1}^{d}||W_i||_{2}^{2}\sum_{i=1}^{d}\frac{||W_i||^{2}_{F}}{||W_i||_{2}^{2}}}{\gamma^2m}}\right)
\]
where $B,d,h>0$, $f_w:X_{B,n} \rightarrow \mathbb{R}^k$ is a d-layer feed forward neural network with ReLu activations, $m$ is the size of the training set and $\alpha$ is the maximum number of units in a layer. Another margin bound based approach uses a metric called spectral complexity, $R_w$ and results in the following bound:
\[
\sim{O}\left(\frac{||X||_2R_w}{\gamma N}log(max_{i}h_{i})+\sqrt{\frac{1}{N}}\right)
\]
where $||X||_2 = \sqrt{\sum_{i}||x_i||_2^2}$, and $max_i h_i$ represent the max number of units in any layer.\cite{bartlettFT17} Another work \cite{aroracompression18}, took a different approach and compared to the previous margin-based approaches, had the closest estimate of the number of parameters in different deep neural networks. In \cite{aroracompression18} the authors use a compression approach with the following definition of $(\gamma,S)-compressible$:
Let $f$ be a classifier and $G_A=\{g_A|A \in \mathbb{A}\}$ be a class of classifiers. $f$ is $(\gamma,S)-compressible$ via $G_A$ if there exists $A \in \mathbb{A}$ such that for any $x \in S$, for all $y$ $f(x)[y]-g_{A}(x)[y] \leq \gamma$. There is a similar definition for $(\gamma,S)-compressible$ with helper string, $s$ where $G_A$ is replaced with $G_{A,s}={g_{A,s}|A \in \mathbb{A}}$, where $G_{A,s}$ is a class of classifiers indexed by trainable parameters and fixed string $s$. The generalization bound states that if there is a trained classifier $f$ that is $(S,\gamma)-compressible$ via $G_{A,s}={g_{A,s}|A \in \mathbb{A}}$ with helper string $s$ where $S$ is a training set with $m$ samples and $A$ is a set of $q$ parameters with at most $r$ discrete values, then the generalization error will be less than or equal to $O\left(\sqrt{\frac{q log r}{m}}\right)$.
Instead of looking at trying to measure the complexity of the hypothesis space, another set of works develop generalization bounds based on the learning algorithm used. In \cite{bousquet02}, various notions of stability are used to create generalization bounds. The stability of an algorithm refers to how the output of a learning algorithm changes when one or more training examples are left out. The strongest form of stability in \cite{bousquet02} is uniform stability, which states that the output of the learning algorithm changes less than some value $\beta$ for all training examples in all possible training sets. When a learning algorithm has uniform stability $\beta$ for a loss function $l$ such that $0 \leq l(A_S,z) \leq M$ for all $z \in \mathbb{Z}$ and for all $s \in \mathbb{S}$, then for any training set size $m \geq 1$ and any $\delta \in (0,1)$ the generalization error is less than or equal to:
\[
2\beta + (4m\beta+M)\sqrt{\frac{ln \frac{1}{\delta}}{2m}}
\]
There has been work done showing that in several different settings, stochastic gradient descent is a stable learning algorithm. \cite{HardtRS15, KuzborskijL17}
The robustness of learning algorithms, or how much the loss value changes with respect to the input space is another property that has been used to develop generalization bounds. If a learning algorithm is $(K,\zeta)$ robust (which means that the input space can be divided into $K$ partitions and that the loss values between the partitions do not differ by more than $\zeta$) then the following generalization error holds:
\[
\zeta(S) + M\sqrt{\frac{2Kln2+2ln\frac{1}{\delta}}{m}}
\]
where $M$ is the largest loss value and $m$ is the number of training examples. \cite{xu10}

There has also been empirical work related to generalization error using a variety of methods. Some empirical work directly measures generalization error. A large scale study was done across multiple domains that looked at how generalization error changes with respect to training size. The experiments showed that the relationship between generalization error and training size is generally $\epsilon = \alpha m^{\beta_g} + \gamma$ where $m$ is the number of training examples. The value of the exponent ($\beta_g$) varied across domains and the paper stated that the exponents must be determined empirically. (insert reference) 
Other empirical work focuses on various methods to improve accuracy and generalization. In Computer Vision, there has been much success in using pre-training though some recent work suggests that ImageNet pre-training only speeds up convergence and does not improve accuracy nor regularization. \cite{he2019rethinking} Excellent performance has been seen in transfer learning: pre-training on a large data set and then fine tuning for a particular task. \cite{Kolesnikov2019BigT} Data set size is another metric investigated empirically. Even when the data set is small, deep networks performed well using pre-training and then fine tuning. \cite{Kolesnikov2019BigT} Experiments showed that `performance on vision tasks increases logarithmically based on volume of training data size'.\cite{SunSSG17} The last set of empirical work involves improving optimization which is important in training neural networks. One technique called gradient centralization has been shown experimentally to improve generalization by regularizing `both the weight space and output space.'\cite{Yong2020GradientCA} The Lookahead Optimization algorithm improves learning stability and lower the variance of the inner optimizer without significantly increasing computation and memory. \cite{Zhang2019LookaheadOK} As discussed above, stable learning algorithms have theoretically determined generalization bounds.


==> figs/effect_of_depth.tex <==
\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics{imgs/depth_ft.pdf}
        \caption{Finetuning}
        \label{fig:depth_pretr_ft}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics{imgs/depth_linear.pdf}
        \caption{Linear}
        \label{fig:depth_pretr_linear}
    \end{subfigure}
\caption{\textbf{Effect of depth.}}
\label{fig:exp_different_depth}
\end{figure*}

==> figs/effect_of_ensemble.tex <==
\begin{figure}[h]
\includegraphics[width=0.9\linewidth]{imgs/ensemble.pdf}
\caption{\textbf{Effects of ensemble.}}
\label{fig:exp_ensemble}
\end{figure}

==> figs/effect_of_width.tex <==
\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{imgs/width_ft.pdf}
        \caption{Finetuning}
        \label{fig:width_pretr_ft}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{imgs/width_linear.pdf}
        \caption{Linear}
        \label{fig:width_pretr_linear}
    \end{subfigure}
\caption{\textbf{Effect of network width.}}
\label{fig:exp_different_width}
\end{figure*}

==> figs/fig_combined_curves.tex <==

%

\begin{figure}[ht]
    \captionsetup[subfigure]{font=footnotesize,labelfont=scriptsize}
    \centering
    % arch
    \begin{subfigure}[t]{0.31\linewidth}
        \includegraphics[width=\textwidth]{imgs/arch_in2cifar.pdf}
        \caption{\label{fig:arch} Architecture: finetune}
    \end{subfigure}
    %pre-train / fine-tune 
    \begin{subfigure}[t]{0.31\linewidth}
        \includegraphics[width=\textwidth]{imgs/pretr_in2cifar.pdf}
        \caption{Transfer: ImageNet to Cifar100}
        \label{fig:imagenet_to_cifar}
    \end{subfigure}
    \begin{subfigure}[t]{0.31\linewidth}
        \includegraphics[width=\textwidth]{imgs/pretr_in2places.pdf}
        \caption{Transfer: ImageNet to Places365}
        \label{fig:imagenet_to_places}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{0.31\linewidth}
        \includegraphics[width=\textwidth]{imgs/pretr_in_places_moco2cifar.pdf}
        \caption{Pretraining: test on Cifar100}
        \label{fig:exp_different_pretrained_models}
    \end{subfigure}
    % depth
    \begin{subfigure}[t]{0.31\linewidth}
        \includegraphics[width=\textwidth]{imgs/depth_ft.pdf}
        \caption{Depth: finetune}
        \label{fig:depth_pretr_ft}
    \end{subfigure}
    \begin{subfigure}[t]{0.31\linewidth}
        \includegraphics[width=\textwidth]{imgs/depth_linear.pdf}
        \caption{Depth: linear}
        \label{fig:depth_pretr_linear}
    \end{subfigure}
    \\
    % ensemble
    \begin{subfigure}[t]{0.31\linewidth}
        \includegraphics[width=\textwidth]{imgs/ensemble.pdf}
        \caption{Ensemble: finetune}
        \label{fig:exp_ensemble}
    \end{subfigure}
    % width
    \begin{subfigure}[t]{0.31\linewidth}
        \includegraphics[width=\textwidth]{imgs/width_ft.pdf}
        \caption{Width: finetune}
        \label{fig:width_pretr_ft}
    \end{subfigure}
    \begin{subfigure}[t]{0.31\linewidth}
        \includegraphics[width=\textwidth]{imgs/width_linear.pdf}
        \caption{Width: linear}
        \label{fig:width_pretr_linear}
    \end{subfigure}
    \\
    % data augmentation
    \begin{subfigure}[t]{0.31\textwidth}
        \includegraphics[width=\textwidth]{imgs/aug.pdf}
        \caption{Data aug: test on Places365}
        \label{fig:aug}
    \end{subfigure}
    % dataset
    \begin{subfigure}[t]{0.31\textwidth}
        \includegraphics[width=\textwidth]{imgs/dataset_ft.pdf}
        \caption{Datasets: effect of finetuning}
        \label{fig:datasets_ft}
    \end{subfigure}
    \begin{subfigure}[t]{0.31\textwidth}
        \includegraphics[width=\textwidth]{imgs/dataset_pretr.pdf}
        \caption{Datasets: effect of pretraining}
        \label{fig:datasets_pr}
    \end{subfigure}
    %\begin{subfigure}[t]{0.31\textwidth}
    %    \includegraphics[width=\textwidth]{imgs/aug_no_pretr_ft.pdf}
    %    \caption{Data aug: no pretrain, finetune}
    %    \label{fig:aug_nopretr_ft}
    %\end{subfigure}
    %\begin{subfigure}[t]{0.31\textwidth}
    %    \includegraphics[width=\textwidth]{imgs/aug_pretr_ft.pdf}
    %    \caption{Data aug: finetune}
    %    \label{fig:aug_pretr_ft}
    %\end{subfigure}
    %\begin{subfigure}[t]{0.31\textwidth}
    %    \includegraphics[width=\textwidth]{imgs/aug_pretr_linear.pdf}
    %    \caption{Data aug: linear}
    %    \label{fig:aug_pretr_linear}
    %\end{subfigure}
    
    \caption{
    \label{fig:combined_plots}
    \textbf{Learning Curves:} See text for description and discussion.
    %\textbf{Learning Curves:} Each plot shows the percent error as the y-axis and $1/\sqrt(n)$ as the x-axis, with $n$ values in parentheses showing the number of samples per class (unless noted otherwise). The y-intercept is asymptotic error at $n=\infty$. %The curve is unbounded at the right side, but we use a minimum of 25 training samples per class because small training sample sizes lead to high variance on test error and inaccuracies due to upper-bounded chance error. 
    %Unless noted, all tests are on Cifar100 with pretraining on ImageNet. Comparison on linear (training only classification layer) highlights the quality of features learned in pretraining.
    }
\end{figure}




==> figs/linear_approx.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{imgs/linear_approx.pdf}
    \vspace{-0.3in}
    \caption{
    \label{fig:linear_approx}
    \textbf{Characterizing a learning curve in terms of error ($e_N$) and data-reliance ($\beta_N$).}
    \vspace{-0.1in}
    }
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> tab/bounds.tex <==
\begin{table*}[h!]
\caption{\textbf{Generalization bound examples:} The bounds each predict generalization error increasing as a function of $n^{-0.5}$. Note: variable notation is consistent only within each line, except $n$.}
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcc}
\toprule
\textbf{Work} & \textbf{Key Variables} & \textbf{Bound} \\
\midrule
\cite{neyshabur2018a} & network depth $d$ & $O\left(n^{-0.5}Bd\sqrt{h\ln(dh)\pi_{i=1}^{d}||W_i||_{2}^{2}\sum_{i=1}^{d}\frac{||W_i||^{2}_{F}}{||W_i||_{2}^{2}}}/\gamma\right)$ \\
\cite{bartlettFT17} & spectral complexity $R_w$ & $O\left(\frac{||X||_2R_w}{\gamma \cdot n}\log(\max_{i}h_{i})+n^{-0.5}\right)$ \\
\cite{aroracompression18} & \makecell{compressibility to $q$ parameters \\with $r$ discrete values} & $O\left(n^{-0.5}\sqrt{q \log r}\right)$ \\
 \cite{bousquet02} & \makecell{based on analysis of stability with margin $\gamma$} & $O\left(n^{-0.5}/\gamma \right)$ \\%where $e_{train}$ is empirical train error and $c$ and $d$ represent multivariate terms that depend on the classification or regression algorithm.
\bottomrule
\end{tabular}
}
\end{center}
\label{tab:bounds}
\end{table*}

==> tab/curve_params.tex <==
\begin{table}[t]
\caption{\textbf{Learning curve parameterization.} We evaluate the effect of estimating different learning curve parameters ($\alpha+\eta n^\gamma + \delta n^{2\gamma}$) on the leave-one-size-out error. \best{Best} results are highlighted.}
\begin{center}
\begin{tabular}{l|r|lllll}
\textbf{Estimated Param} & \textbf{Fixed Param} & \textbf{25} & \textbf{50} & \textbf{100} & \textbf{200} & \textbf{400} \\
\midrule
$\alpha, \eta$ & $\gamma=-0.5, \delta=0$          & 4.16        & \best{0.71}        & 0.6          & 0.57         & 1.09         \\
$\alpha, \eta, \gamma$ & $\delta=0$ & \best{2.24}        & 0.79        & \best{0.53}         & \best{0.53}         & \best{0.85}         \\
$\alpha, \eta, \gamma, \delta$ &  &  3.12        & 0.86        & 0.63         & 0.61         & 1.04        
\end{tabular}
\end{center}
\label{tab:model_choice}
\end{table}

==> tab/weights.tex <==
\begin{table}[t]
\caption{\textbf{Weighting and model parameterization: } In brief, these results indicate that the two-parameter model explains at least 98.9\% of test error variance for most curves and achieves similar RMSE to more complex models, while the weighting encourages better fit for models with more training samples.  %\best{Best} and \sbest{second best} results are highlighted.
Median $R^2$ statistic across learning curves is shown. RMSE and NLL are computed for leave-one-size-out (e.g. omit all models trained with 25 samples when predicting their error based on the other models trained with different numbers of samples). NLL (negative log likelihood) reflects the average log probability of the test error for each model, according to the learning curve expectation and variance. P-values from paired two-sided t-tests reflect significance of difference between other models and our preferred model/weighting in the top row.  This weighting intentionally biases toward fitting the larger-sample models to provide more accurate asymptotic error predictions, and our results suggest lower average RMSE and NLL for 400-sample models. Differences in RMSE between models and weighting are not statistically significantly different, but the other models/weights confidently outperform in NLL. 
}
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccccccccccccc}
\toprule
& & & \multicolumn{7}{c}{RMSE} & \phantom{abc} & \multicolumn{7}{c}{NLL} \\
\cmidrule{4-10}  \cmidrule{12-18}
\textbf{Params} & \textbf{Weights} & $R^2$  & \textbf{25} & \textbf{50} & \textbf{100} & \textbf{200} & \textbf{400} & \textbf{avg} & \textbf{p-value} & & \textbf{25} & \textbf{50} & \textbf{100} & \textbf{200} & \textbf{400} & \textbf{avg} & \textbf{p-value} \\
\midrule
\multirow{3}{}{$\alpha,\eta$} 
& $\frac{1}{\sigma_i^2F_i}$ & 0.989 & 3.22 & 1.26 & 0.69 & 0.63 & 1.31 & 1.42 & - & & 5.58 & 4.1  & 4.21 & 1.84 & 3.27 & 3.80 & - \\
& $\frac{1}{\sigma_i^2}$ & 0.990 & 2.97 & 1.45 & 0.50 & 0.64 & 1.78 & 1.47 & .10 &  & 4.45 & 4.45 & 2.51 & \best{1.19} & 3.97 & 3.31 & .02 \\
& $1$ & 0.985 & 2.92 & 1.44 & \best{0.42} & 1.14 & 2.23 & 1.63 & .16 &  & 4.11 & 4.36 & 2.06 & 1.56 & 4.46 & 3.31 & .03  \\
\cmidrule{1-18}
$\alpha, \eta, \gamma$
& $\frac{1}{\sigma_i^2F_i}$ & 0.998 & \best{2.27} & 0.84 & 0.55 & \best{0.54} & \best{0.81} & \best{1.00} & .31 &  & 3.61 & 2.49 & 3.31 & 1.44 & 1.39 & 2.45 & $<$.001  \\
\cmidrule{1-18}
$\alpha, \eta, \delta$
& $\frac{1}{\sigma_i^2F_i}$ & 0.999 & 2.81 & \best{0.73} & 0.63 & 0.56 & 0.90 & 1.13 & .50 &  & \best{2.49} & \best{1.55} & \best{1.70} & 1.44 & \best{1.33} & \best{1.70} & $<$.001 \\
\cmidrule{1-18}
$\alpha, \eta, \delta, \gamma$
& $\frac{1}{\sigma_i^2F_i}$ & 0.999 & 3.09 & 0.86 & 0.65 & 0.61 & 1.07 & 1.26 & .34 &  & 2.61 & 1.84 & 1.71 & 1.65 & 1.42 & 1.85 & $<$.001 \\
\bottomrule
\end{tabular}
}
\end{center}
\label{tab:weights}
\end{table}
